A Data-Centric Multi-Objective Learning Framework for Responsible Recommendation Systems

Recommendation systems effectively guide users in locating their desired information within extensive content repositories. Generally, a recommendation model is optimized to enhance accuracy metrics from a user utility standpoint, such as click-through rate or matching relevance. However, a responsible industrial recommendation system must address not only user utility (responsibility to users) but also other objectives, including increasing platform revenue (responsibility to platforms), ensuring fairness (responsibility to content creators), and maintaining unbiasedness (responsibility to long-term healthy development). Multi-objective learning is a potent approach for achieving responsible recommendation systems. Nevertheless, current methods encounter two challenges: difficulty in scaling to heterogeneous objectives within a unified framework, and inadequate controllability over objective priority during optimization, leading to uncontrollable solutions. In this paper, we present a data-centric optimization framework, MoRec, which unifies the learning of diverse objectives. MoRec is a tri-level framework: the outer level manages the balance between different objectives, utilizing a proportional-integral-derivative (PID)-based controller to ensure a preset regularization on the primary objective. The middle level transforms objective-aware optimization into data sampling weights using sign gradients. The inner level employs a standard optimizer to update model parameters with the sampled data. Consequently, MoRec can flexibly support various objectives while maintaining the original model intact. Comprehensive experiments on two public datasets and one industrial dataset showcase the effectiveness, controllability, flexibility, and Pareto efficiency of MoRec, making it highly suitable for real-world implementation.

==> sections/method-old.tex <==
\section{Methodologies}
\subsection{Tri-level Framework}
% 
In summary, our MoRec presents a tri-level framework designed to address the challenges of balancing various objectives, illustrated in \textcolor{red}{Figure}. The framework comprises three interconnected levels that collaborate harmoniously, ensuring an efficient and effective process. 

\begin{itemize}[leftmargin=*]
\item \textbf{Outer-level - Objective Controller}: The objective controller functions as a guiding mechanism, steering the overall optimization by monitoring and adjusting objectives to achieve a desired balance and performance.
\item \textbf{Middle-level - Adaptive Data Sampler}: The adaptive data sampler is in charge of dynamically selecting appropriate training samples to optimize the corresponding objectives. This component offers a unified approach for optimizing diverse objectives while overcoming the limitations of conventional methods.
\item \textbf{Inner-level - Standard Model Optimizer}: The standard model optimizer remains unaltered, i.e. SGD-based optimizer, concentrating on the routine training of the backbone model. This level guarantees that the optimization process does not disrupt the underlying model's structure, stability, or latency.
\end{itemize} 

Together, these three levels form a comprehensive optimization framework that facilitates the seamless integration of various objectives while preserving the model's controllability and optimizing its performance. The overall procedure could be referred to Algorithm~\ref{alg:overall}.

\begin{algorithm}
    \scriptsize
    \KwIn{Training Data ${D}_t$, Valid Data ${D}_v$, Data Sampler $\mathrm{DS}$, Objective Controller $\mathrm{OC}$, Objective Priority $\rho$, Expected Accuracy Loss $\hat{\ell}$}
    \KwIn{Model $M_\theta$}
    {
        Initialize $\mathrm{OC}$ with $\rho$ and $\hat{\ell}$\;
        Initialize sampling weight $\bm{W}$ in $\mathrm{OC}$ with $M_\theta$, ${D}_t$ and ${D}_v$\;
        Get $\mathrm{train\_loader}$ with ${D}_t$ and $\mathrm{DS}$\;
        \Repeat{Convergence or reaching max epoch}
        {
        \For(\hspace{6em}\tcp*[h]{Middel Level: data sampling}){$\mathrm{batch} \in \mathrm{train\_loader}$}
        {
            $\bm{\ell} \gets$ Calculate loss with $M_\theta$\;
            $\bm{\alpha} \gets \mathrm{OC}(\bm{\ell})$ \tcp*{\textit{Outer Level: objective control}}
            $\mathrm{loss} \gets \bm{\alpha}^T \bm{\ell}$\;
            Update $M_\theta$ with $\mathrm{loss}$ \tcp*{\textit{Inner Level: model optimization}}
        }
        Update sampling weight $\bm{W}$ in $\mathrm{DS}$ \tcp*{\textit{sampling weight optimization}}
        }
    }
    \caption{The Tri-level Framework MoRec.}
    \label{alg:overall}
\end{algorithm}

\subsection{Adaptive Data Sampler}
The first challenge in multi-objective optimization is how to model multiple objectives. In previous multi-objective optimization works, many approaches involve designing specific loss functions related to the objectives, guiding the model to optimize towards the specified goals. These methods rely on intricate design and do not have scalability across different model structures or data distributions. Moreover, due to the heterogeneity of loss functions, the gradients brought by different loss functions requires special designs when merging, such as MGDA. We propose an adaptive data sampler to achieve unified multi-objective modeling from the data perspective.
  
The basic idea of our data sampler comes from a simple concept: the importance of each sample under different objectives varies. For example, to improve the model's performance in terms of revenue, items with higher profits should have a higher probability of being recommended. Therefore, the corresponding sample weights should be higher. Giving the accuracy-dominated loss function $l_{acc}(\cdot)$, the weighted loss value for a certain objective can be represented as $L=\sum_{i=0}^{N}w_i\cdot l_{acc}(x_i), w_i\ge0\; \text{and} \; \sum_{i=1}^{N}w_i=1$. Here $w_i$ denotes the weight for the objective corresponding to the sample $x_i=(u_i,e_i)$. This formula can be transformed into $L=\mathbb{E}_{x\sim P_w}\,l(x)$, meaning that the weighted loss value can be calculated by sampling the data according to the distribution $P_w(i)=w_i$. Therefore, our problem becomes optimizing the data sampling weight for each objective. 
   
Based on this idea, we designed an adaptive data sampling method to replace the complex loss function design by selecting appropriate samples for optimizing each objective. This approach allows us to avoid designing additional loss functions for the objectives and unifies modeling each objective as the accuracy-dominated loss function $l_{acc}(\cdot)$. Therefore, it provides a plug-and-play data sampler without modifying the training process. Next, we demonstrate the optimization of the sampling weight $\mathbf{w}=\{w_i\}$ for the accuracy, fairness, alignment, and revenue objectives.  
   
\subsubsection{Accuracy} For the Accuracy objective, we maintain the same sampling strategy as used during the model optimization focused on accuracy, i.e., uniform sampling, with fixed sampling weights $w_i=\frac{1}{|D|}$. The theory behind is the same as it in optimizing revenue objective, i.e. Eq~\ref{eq:opt_rev}.

\subsubsection{Revenue} For the revenue objective, the optimal sampling weight $\mathbf{w}$ could be obtained easily by solve the following linear programming problem. 
\begin{equation}
\begin{split}
    \mathbf{w} = \arg\max_{\mathbf{w}} \mathcal{O}_{rev} 
    &=\arg\max_{\mathbf{w}} \sum_{i=1}^{|D|} w_i\cdot r(e_i)\cdot l_{acc}(x_i)\\
\text{subject to}\;
&\sum_{i=1}^{|D|}w_i=1,\, w_i\ge 0
\end{split}
\label{eq:opt_rev}
\end{equation}

The optimal solution to the problem is $w_i\sim r(e_i)$, regarding the $l_{acc}(\cdot)$ as constant when optimizing $\mathbf{w}$.

\subsubsection{Fairness} For the fairness objective, we designed a signed-SGD weight adjustment scheme for the Least Misery objective in ~\ref{eq:fair}. 

\begin{equation}
\begin{split}
\mathbf{w} &= \arg\max_{\mathbf{w}} \mathcal{O}_{fai} \\
&= \arg\max_\mathbf{w} \min_z \{-\mathcal{L}^{(z)}(w_z), \forall z \in  \mathcal{Z} \}\\
&= \arg\min_\mathbf{w} \max_z \{\mathcal{L}^{(z)}(w_z), \forall z \in  \mathcal{Z} \}
\end{split}
\end{equation}
where
\begin{equation*}
    \mathcal{L}^{(z)}(w_z) = -w_{z}\sum_{x\in D_z}l_{acc}(x)
\end{equation*}

Assume $\mathcal{L}^{(z^*)}(w_{z^*})=\max_z \mathcal{L}^{(z)}(w_z)$, which means $z^*$ is the group with the highest loss value. Since $\mathcal{L} > 0$, the signed gradient calculation can be defined as follows:
\begin{equation}
sign\left(\frac{\partial{\mathcal{O}_{fai}}}{\partial w_z}\right) =  
\begin{cases}  
    0, \; & i\neq z^* \\  
    1, \; & i=z^*  
\end{cases}
\end{equation}

This means that the sampling weight of the group with the highest loss should increase, while the weights of other groups remain unchanged. 

\subsubsection{Alignment} For the objective, the samples with larger weights during the optimization process will intuitively have higher exposure probability in the recommendation. We assume that the sample weight $w_i$ for $x_i$ is positively correlated with $P(x_i)$, i.e., $sign\left(\frac{\partial P(x_i)}{\partial w_i}\right)=1$. According to Eq~\ref{eq:align}, we have:  

\begin{equation*}
\frac{\partial \mathcal{O}_{ali}}{\partial P(x_i)}=\log{\frac{Q(x_i)}{P(x_i)}}
\end{equation*}
Thus, we can obtain the sign gradient:  
\begin{equation}
sign\left(\frac{\partial \mathcal{O}_{ali}}{\partial P(x_i)}\right)=\mathbb{I}\left(Q(x_i)-P(x_i)\right)=  
\begin{cases}  
    1, \; & P(e_i)< Q(e_i) \\  
    0, \; & P(e_i)=Q(e_i) \\  
    -1, \; & P(e_i)>Q(e_i)  
\end{cases}
\end{equation}
where $\mathrm{I}(\cdot)$ is the sign function. Hence the composite sign gradient is:

\begin{equation}
sign\left(\frac{\partial \mathcal{O}_{ali}}{\partial w_i}\right)=sign\left(\frac{\partial \mathcal{O}_{ali}}{\partial P(x_i)}\cdot \frac{\partial P(x_i)}{\partial w_i}\right)=\mathbb{I}\left(Q(x_i)-P(x_i)\right)
\end{equation}

Intuitively, in the item recommendation list predicted by the model, the sampling weights of items with a exposure volume lower than the specified value should increase, and vice versa.  
   
In both fairness and alignment objectives, the optimization of sampling weights needs to be guided by the indicators of the model's current state. Inspired by works in meta learning [3], we use the model's performance on the validation set to guide the update of sampling weights $\mathbf{w}$. During training, we construct multiple batches by sampling with objective-related weights, and then use the unifies loss function $l_{acc}(\cdot)$ to calculate the loss for each objective, thereby obtaining multiple gradients. Note that although retaining a weight for each sample can achieve more fine-grained optimization, it would introduce unacceptable complexity in the weight optimization and data sampling processes. Therefore, we employ a clustering strategy for each objective, where samples with similar contribution to the objective are clustered in to one group and share share the sampling weight. For example, for the revenue objective, we divide samples into groups according to the profit of item, with equal sampling weights within each group. The clustering strategies for other objectives are shown in Section~\ref{sec:exp}.

\subsection{PID-based Objective Controller}
After unifying the modeling of multiple objectives using the data sampling-based method, we can obtain gradient for different objectives. How to synthesize these gradients to determine the final update direction of the model parameters is another challenge in multi-objective optimization. 

Scalarization is a very common scheme, which linearly weights the gradients to obtain the final gradient. However, it is inevitable that when multiple gradients are combined, the gradient information corresponding to different objectives may conflict. Therefore, selecting appropriate coefficients to obtain a relatively optimal synthetic gradient information is important. A common practice is to manually adjust the coefficients, but the time cost is relatively high; other works combine the SGD algorithm and use the KTT conditions to solve a set of coefficients adaptively, such as MGDA. However, these methods lack consideration for the controllability of multi-objective optimization, which means the model's performance . Subsequent algorithms derived from MGDA, such as PEMTL and EPO, have additional designs for multi-objective control, but their control only achieves preference control on different objectives, which is not very suitable for recommendation systems.  
   
In recommendation systems, we believe that the controllability of multi-objective optimization needs to satisfy two aspects: first, \textbf{to ensure that the most important accuracy of the recommendation model is not compromised (\textit{Property 1})}, and second, \textbf{the model's preference on other objectives can be artificially controlled (\textit{Property 2})}. With these two controllable properties, the designers of the recommendation system can optimize the model according to the platform's requirements to set the target bias and make its performance better on specific targets, without worrying about the accuracy of the optimized model being greatly reduced. To achieve these two controllability, we designed a PID-based objective controller.  
   
PID is a common feedback loop component in industrial control applications, whose purpose is to control a certain performance parameter of the system to a predetermined reference value. This goal aligns with our aim to maintain the model's accuracy (property 1). The standard PID consists of Proportional, Integral and Derivative parts, which capture the current error, past error, and future error respectively. We use P and I parts. First, we decouple the weight of the gradient corresponding to accuracy from other objectives and synthesize the gradient in the following form:  
   
\begin{equation}  
\vec{g}_{\text{final}}=\alpha_{\text{acc}}\cdot \vec{g}_{\text{acc}} + \lambda \cdot \sum_{\text{obj}\neq \text{acc}} \alpha_{\text{obj}} \cdot \vec{g}_{\text{obj}}  
\end{equation}  
   
Where $\alpha_{\text{obj}}$ represents the weight corresponding to the gradient $\vec{g}_{\text{obj}}$ of the objective $\text{obj}$, and $\lambda$ is a constant. Inspired by paper [1], we regard the loss value of the accuracy objective as the monitor performance metric to be controlled. The control signal output by the PI controller serves as the weight $\alpha_{\text{acc}}$ of the gradient corresponding to accuracy. The preset loss value $l_0$ is the final loss value under single-objective optimization. If the loss value of the model at time $t$ is $l_t$, then:  
   
\begin{equation}  
\alpha_{\text{acc}}(t)=\frac{K_p}{1+\exp(err(t))} - K_i \sum_{j=1}^t err(j) + \alpha_{\text{min}}  
\end{equation}  
   
Where $err(t)=l_0-l_t$ represents the error at time $t$, $K_p, K_i$ represent the coefficients of the proportional and integral parts, respectively, and are non-negative values. $\alpha_{\text{min}}$ is the set minimum value.  
   
Under this setting, when $err(t)$ is positive and increasing, the first term becomes smaller until it approaches 0, the second term is also decreasing, causing $\alpha_{\text{acc}}(t)$ to decrease. This is because the preset performance has been reached, so a lower weight is given to accuracy; on the contrary, when $err(t)$ is negative and the absolute value is small enough, the first term approaches the maximum value $K_p$, the second term is also increasing, causing $\alpha_{\text{acc}}(t)$ to increase. This is because the model's accuracy performance is lower than the preset value, so a higher weight is given to accuracy. In this way, the accuracy performance of the model will stabilize near the preset value, thus controlling the accuracy of the model without decreasing.  
   
As for property 2, we aim to control the model's preferences priority toward other objectives except the accuracy by giving a priority vector $\mathbf{\rho}$. Thanks to our previous data sampling method to unify the modeling of various objectives, the resulting loss and gradient are homogeneous (they are calculated by the same function and of the same order of magnitude in terms of loss values and gradient values). By setting $\alpha_{\text{obj}} \propto\rho_{\text{obj}}$, we can achieve an excellent objective priority control effect, which we further verify in subsequent experiments.



